Weighted-Lasso for Structured Network Inference from Time Course Data

We present a weighted-Lasso method to infer the parameters of a first-order vector auto-regressive model that describes time course expression data generated by directed gene-to-gene regulation networks. These networks are assumed to own a prior internal structure of connectivity which drives the inference method. This prior structure can be either derived from prior biological knowledge or inferred by the method itself. We illustrate the performance of this structure-based penalization both on synthetic data and on two canonical regulatory networks, first yeast cell cycle regulation network by analyzing Spellman et al's dataset and second E. coli S.O.S. DNA repair network by analysing U. Alon's lab data.

==> appendices.tex <==
\section{Proof of Proposition \ref{prop:var1_mle}}\label{app:proof1}

Thanks to the Markov property of $X_t$, the likelihood writes
\begin{equation}
  \mathcal{L}(\mathbf{X}) = \mathbb{P}(X_0) \prod_{t=1}^n \mathbb{P}(X_t|X_{t-1}).
\end{equation}

Assume for  the sake  of simplicity, yet  with no loss  of generality,
that $\mathbf{b}  = 0$ and $\mathbf{D}=I_p$.  Since  $X_t$ is governed
by                    \eqref{eq:autoregressive}                    and
$\varepsilon_t\sim\mathcal{N}(0,I_p)$, then
\begin{equation*}
  X_t | X_{t-1} = x \sim \mathcal{N}\left(x\mathbf{A}, I_p \right).
\end{equation*}
Hence,  according  to the  parameters  of  interest $\mathbf{A}$,  the
log-likelihood turns to
\begin{equation*}
  \log \mathcal{L}(\mathbf{X};\mathbf{A}) = C-\frac{1}{2}
  \sum_{t=1}^n \left(    X_t-    X_{t-1}\mathbf{A}\right)^\intercal
  \left( X_t- X_{t-1}\mathbf{A} \right), 
\end{equation*}
where  $C$ does  not  depend  on $\mathbf{A}$.   Using  the fact  that
$\mathbf{a}\mathbf{b}^\intercal                                       =
\mathrm{Tr}(\mathbf{a}\mathbf{b}^\intercal)                           =
\mathrm{Tr}(\mathbf{b}^\intercal\mathbf{a})$   for   $\mathbf{a}$  and
$\mathbf{b}$ column vectors and that  the trace operator is linear, it
writes
\begin{equation*}
  \log \mathcal{L}(\mathbf{X};\mathbf{A}) = C'+\frac{1}{2}\left\{
    2 \mathrm{Tr}\left(\sum_{t=1}^n X_t^\intercal X_{t-1} \mathbf{A}\right) -
    \mathrm{Tr}\left(                   \mathbf{A}^\intercal\sum_{t=1}^n
      X_{t-1}^\intercal X_{t-1} \mathbf{A} \right)\right\}.
\end{equation*}
By  means  of notation  \eqref{eq:variances},  we  get the  equivalent
maximization   problem   \eqref{eq:max_log-likelihood}.    Then,   the
maximum-likelihood estimator (MLE) $\widehat{\mathbf{A}}^\mathrm{mle}$
is obtained by direct differentiation, remembering the differentiation
rules for the trace operator:
\begin{equation*}
  \frac{\partial}{\partial   \mathbf{A}}   \mathrm{Tr}   (\mathbf{V}^{\intercal}
  \mathbf{A})    =    \mathbf{V},   \qquad    \frac{\partial}{\partial
    \mathbf{A}} \mathrm{Tr} (\mathbf{A}^\intercal \mathbf{S} \mathbf{A})
  = 2\mathbf{S}\mathbf{A}.
\end{equation*}
since $\mathbf{S}$ is  symmetric.  Null-gradient condition and problem
concavity leads to the final result.

% This reduces to
% \begin{equation*}
%   \log \mathcal{L}(\mathbf{X};\mathbf{A}) = C'+\frac{1}{2}
%   \sum_{t=1}^n \left(  X_t^\intercal X_{t-1}\mathbf{A} + X_t^\intercal
%     X_{t-1}\mathbf{A} -
%     \mathbf{A}^\intercal X_{t-1}^\intercal  X_{t-1}\mathbf{A} \right).
% \end{equation*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "J2C.tex"
%%% End:


